Principles Of Heliophysics: a textbook on the universal processes behind planetary habitability

Heliophysics is the system science of the physical connections between the Sun and the solar system. As the physics of the local cosmos, it embraces space weather and planetary habitability. The wider view of comparative heliophysics forms a template for conditions in exoplanetary systems and provides a view over time of the aging Sun and its magnetic activity, of the heliosphere in different settings of the interstellar medium and subject to stellar impacts, of the space physics over evolving planetary dynamos, and of the long-term influence on planetary atmospheres by stellar radiation and wind. Based on a series of NASA-funded summer schools for early-career researchers, this textbook is intended for students in physical sciences in later years of their university training and for beginning graduate students in fields of solar, stellar, (exo-)planetary, and planetary-system sciences. The book emphasizes universal processes from a perspective that draws attention to what provides Earth (and similar (exo-)planets) with a relatively stable setting in which life as we know it could thrive. The text includes 200 "Activities" in the form of exercises, explorations, literature readings, "what if" challenges, and group discussion topics; many of the Activities provide additional information complementing the main text. Solutions and discussions are included in an Appendix for a selection of the exercises.

==> chapters/mhd/commonprinciples.tex <==
\section{Impulsive events in review: common principles}
Energetic events related to the magnetic field of the Sun and of the planets share the fundamentals of physics everywhere: in analyzing them, we focus on the budgets and flows of energy (through sources, reservoirs, and sinks), to the conditions required for rapid energy conversion between the reservoirs of magnetic energy, of kinetic energy (bulk, thermal, and energetic particles), and of electromagnetic energy (photons or wave phenomena in the magnetic field), with a small (and often neglected) role for gravitational potential energy. Solar flares, coronal mass ejections, and magnetospheric storm phenomena are all consequences of large and rapid increases in conversion of energy from the magnetic reservoir into other forms, often (it is commonly assumed) involving enhanced magnetic reconnection that itself frequently is involved in a loss of equilibrium.

In the solar atmosphere as in planetary magnetospheres the main source of energy is the advection (in terrestrial physics often called 'convection') of magnetic field. For the Sun, that is mainly flux emergence through the solar surface in combination with the displacement of field across the surface by plasma winds (commonly referred to as 'flows' by astrophysicists). In planetary magnetospheres that is a combination of the incoming field and, primarily, the momentum of the solar wind, as well as the movement of the planetary magnetic field with the atmosphere of the planet. 

The most important energy loss terms, or sinks, for the energy stored in the magnetic field that are commonly associated with any impulsive event on the Sun and in planetary magnetospheres include collisional heating, charged-particle precipitation onto the lower atmosphere, and electromagnetic radiation. Solar and planetary events differentiate primarily by energy being lost in bulk kinetic flows (which is an important loss term for solar coronal mass ejections but relatively unimportant in magnetospheric storms), thermal conduction to the lower atmosphere (important for solar events but hardly in terrestrial storms), and the escape of energetic neutral particles (in which energetic ions can escape magnetospheres after neutralizing charge-exchange collisions with planetary atmospheres, but which appears to be an unlikely avenue under solar conditions --~despite the large reservoir of neutral particles around the photosphere).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% QQQ
\begin{figure}[t]
\setlength{\unitlength}{0.8cm}
\begin{picture}(13,10.3)
{\scriptsize
%\graphpaper[1](0,0)(13,10.3)
\thinlines
\put(0.1,6.4){\framebox(2.8,1.5)}

\put(0,6.3){\framebox(3,1.7){
\begin{minipage}{3cm}
\centerline{bulk flow}\centerline{kinetic energy}\centerline{{\em \color{red}[flux emergence]}}
\end{minipage}}}

\put(5,6.5){\framebox(3,1.5){
\begin{minipage}{3cm}
\centerline{magnetic}\centerline{energy}\centerline{(primary)}
\end{minipage}}}

\put(5,3.5){\framebox(3,1.5){
\begin{minipage}{3cm}
\centerline{plasma}\centerline{mechanical energy}
\end{minipage}}}

\put(10,2){\framebox(3,1.5){
\begin{minipage}{3cm}
\centerline{($\sim$) poloidal field}\centerline{magnetic energy}\centerline{(secondary)}
\end{minipage}}}

\put(1.5,4.25){\oval(3,1.5)}

\put(0,3.5){\makebox(3,1.5){
\begin{minipage}{3cm}
\centerline{(heated)}\centerline{atmosphere}
\end{minipage}}}

\put(1.5,1.25){\oval(3,1.5)}

\put(0,0.5){\makebox(3,1.5){
\begin{minipage}{3cm}
\centerline{escaping}\centerline{neutrals}
\end{minipage}}}

\put(6.5,1.25){\oval(3,1.5)}
\put(5,0.5){\makebox(3,1.5){
\begin{minipage}{3cm}
\centerline{electromagnetic}\centerline{radiation}
\end{minipage}}}

\put(11.5,5.75){\oval(3,1.5)}

\put(10,5){\makebox(3,1.5){
\begin{minipage}{3cm}
\centerline{escaping}\centerline{plasma \& field}
\end{minipage}}}

\put(3,7.25){\vector(1,0){2}}\put(5,6.5){\vector(-4,-3){2.2}}\put(5,3.5){\vector(-4,-3){2.2}}

\put(5,4.25){\vector(-1,0){2}}

\put(6.5,6.5){\vector(0,-1){1.5}}\put(8,7.25){\vector(2,-1){2.1}}

\put(8,4.5){\vector(2,1){2}}\put(8,4){\vector(2,-1){2}}

\put(6.5,3.5){\vector(0,-1){1.5}}\put(11.5,3.5){\vector(0,1){1.5}}\put(10,2.5){\vector(-2,1){2}}

\put(10,2.25){\line(-1,0){1.5}}\put(8.5,2.25){\vector(-4,1){5.7}}

\put(4,7.4){I}\put(6.6,5.6){II}\put(9,7){III$_{\,{\color{blue}(sw)}}$}\put(9,5.5){III${}^{\prime}$}

\put(11.6,4.2){\color{blue} (III${{}^{\prime \prime}}_{\,(rot)}$)}\put(9.1,3.5){\color{blue} (IV)}\put(8.3,2.8){\color{blue} (IV${}^{\prime}$)}

\put(8.5,2.3){\color{blue} (IV${}^{\prime \prime}$)}

\put(4,4.4){V}\put(4,2.4){\color{blue} (V${}^{\prime}$)}\put(5.9,2.2){V${}^{\prime \prime}$}

\put(1.5,3.5){\vector(3,-2){3.5}} \put(1.5,2.5){\color{red}[V${}^{\prime \prime}$]}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\put(1.5,6.3){\vector(0,-1){1.3}}\put(1.6,5.5){$0_{\,{\color{blue}(rot)}}$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\put(3,9.4){\oval(6,0.8)}

\put(0,9){\makebox(6,0.8){
\begin{minipage}{6cm}
\centerline{irreversible heating of solar wind}
\end{minipage}}}

\put(1.5,8){\vector(0,1){1}}

\put(1.6,8.4){\color{blue} ($0_{\,(sw)}$)}

\put(4.3,5.6){II${}^{\prime}$}
}\end{picture}
\caption[General energy flow chart for magneto- and ionospheres.]{\label{fig:sumE}(Simplified) general energy flow chart [developed] for planetary
magnetospheres and ionospheres [but here generalized to also apply to the solar atmosphere (with solar-specific processes added in red italics between brackets, and processes generally ignored or ignorable in the solar atmosphere shown in blue between parentheses)].
Rectangular boxes: energy reservoirs. Rounded boxes: energy sinks.
[Arrows]: energy flow/conversion processes. (Note: only the energy-flow
paths are shown,
not the mass-flow paths.) [Modified after Fig.~II:10.4]
}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Energy budget diagram}\label{diagram}

A flow diagram connecting the most important energy reservoirs was developed for magnetospheric phenomena in Sect.~II:10.4.3. The remainder of this section highlights the similarities and differences between magnetospheric and solar phenomena, generalizing the discussion based on that original wording as well as modifying the associated original Fig.~II:10.4. This diagram highlights where substantial differences in the importance of processes occur. For example, electromagnetic radiation from the Sun's surface (the equivalent of a planetary atmosphere) is a large fraction of the overall energy budget of a solar impulsive event but is small for disturbances in planetary magnetospheres where, in contrast, energy carried by escaping neutrals is important. And whereas ring currents and other large kinetic reservoirs are important within the evolving field of magnetospheres, such counterparts are commonly ignored in the energy budget of solar events. 

\ors[II:10.4.3] ``In Fig.\,\ref{fig:sumE}, the primary source of energy ---~bulk-flow kinetic energy, either of the solar wind or of planetary rotation [for magnetospheres, or flux emergence as well as surface flux transport for the solar atmosphere]~--- is shown by the double-lined box. Energy reservoirs are shown by rectangular boxes (with form of energy identified).  Energy sinks, where energy is dissipated or leaves the system, are shown by rounded boxes [\ldots] Energy conversion processes are shown by [\ldots] arrows indicating the direction of energy flow.  The labels on the lines are keyed to the discussion of the corresponding process in the text; subscript $(sw)$ or $(rot)$ --- process [in magnetospheres] important only for dominant solar-wind or dominant rotation source, respectively; no subscript --- important for both.  Processes of minor importance [\ldots] have been left out.

 (1) [In {\em magnetospheres},] {\bf Process I} is the initial conversion of bulk-flow kinetic energy into magnetic energy. With the solar-wind source, the magnetic energy is stored predominantly in the magnetotail.  With the planetary-rotation source, the magnetic energy is stored predominantly in the azimuthal magnetic field, which is in the direction of lagging behind rotation of the planet (like the Parker spiral relative to rotation of the Sun). [In the {\em solar atmosphere} it is the storage of non-potential energy in the atmospheric field, either by emergence of a non-potential field, the interaction of emerging flux with a pre-existing magnetic field, or the buildup of energy by the stressing of the field by large scale flows such as the surface differential rotation, often in combination with random-walk flux dispersal and meridional advection.]

(2) [In {\em magnetospheres},] {\bf Process II} is conversion of magnetic energy into mechanical energy that is then stored in magnetospheric plasma. It includes formation and energization of the plasma sheet (by magnetic reconnection and adiabatic compression) and energization of the plasma in the ring current region (predominantly by adiabatic compression during inward transport; although energy is also removed of course by adiabatic expansion during outward transport, the net effect is energy addition as long as there is a net inflow of plasma, to increase the ring current or maintain it against losses). Additionally, in magnetospheres with a significant interior source of plasma from a moon (Io at Jupiter, Enceladus at Saturn) there is the {\em pick-up} process: ionization of slow-moving (Keplerian) neutrals in the presence of flowing (nearly corotating) plasma, which imparts both flow and thermal energy to the ions. [In the {\em solar atmosphere} this process reflects the heating of the corona and the initial acceleration of the solar wind.]

(3) [In {\em magnetospheres},] {\bf Process II${\null}^{\prime}$} is also conversion of magnetic energy into mechanical energy which, however, goes directly into the ionosphere and the aurora (these are not shown in Fig.\,\ref{fig:sumE} --- as far as the energy budget is concerned, they are simply intermediaries in the process by which magnetic energy is converted to heat of the atmosphere). The process, closely associated with [field-aligned] Birkeland currents, consists primarily of collisional and Joule heating of the ionosphere as well as auroral acceleration and precipitation. [In the {\em solar atmosphere} this process has an equivalent in the heating of the chromosphere through current, waves, and conduction from the corona.]

(4) [In {\em magnetospheres},] {\bf Processes III, III${\null}^{\prime}$, III${\null}^{\prime\prime}$} 
represent the loss of energy (mechanical and magnetic) by
outflow down the distant magnetotail; they all involve magnetic
reconnection, since the magnetic field lines must sooner or later
become disconnected from the planetary dipole. In a rotation-dominated
magnetosphere, processes III${\null}^{\prime}$ and III${\null}^{\prime\prime}$
are related to the formation of the planetary/magnetospheric wind. [In the {\em solar atmosphere}, processes III and III${\null}^{\prime}$] represent those that enable the formation of the magnetized solar wind and, for impulsive phenomena, the processes involved in CMEs. Process~III${\null}^{\prime\prime}$ was likely important in the young, rapidly spinning Sun.]

 (5) [In {\em magnetospheres},] {\bf Processes IV, IV${\null}^{\prime}$} describe energy conversions
between plasma in the inner regions of the magnetosphere (ring
current, plasma torus) and the nearly dipolar but perturbed magnetic
field. Process~IV represents the deformation of the magnetic field by
plasma pressure in the ring current region as well as by corotational
stresses. Process {IV${\null}^{\prime}$}, in turn, represents energization
of the plasma by adiabatic compression during inward transport related
to the distorted poloidal magnetic field (rather than to the
magnetotail field, as in process II; the distinction between the two
is not always clear-cut). [In the {\em solar atmosphere}, these could in principle correspond to the impact on the plasma of expansion and contraction of the coronal magnetic field as it evolves during coronal mass ejections, or conversely of the field by the pressure of the plasma (and MHD waves), but these are relatively minor and not often explicitly discussed.]

(6) [In {\em magnetospheres},] {\bf Process IV${\null}^{\prime \prime}$} is conversion of magnetic energy into heating of the atmosphere, via the ionosphere and the aurora, analogous to process {II${\null}^{\prime}$} but taking energy from the distorted magnetic field in the outer magnetosphere rather than from the magnetotail or the wrapped-up azimuthal field. The related auroral processes may be important for substorm onset. [In the {\em solar atmosphere}, counterparts of this are generally viewed as integrated with the combined pathway II+V.]

(7) {\bf Energy sinks}: loss of magnetic and mechanical energy through processes III, {III${\null}^{\prime}$}, {III${{\null}^{\prime \prime}}$}, {II${\null}^{\prime}$}, and {IV${{}\null^{\prime \prime}}$}] have already been discussed. In addition, mechanical energy of plasma in the {\em magnetosphere} is lost to the atmosphere by particle precipitation [and in the {\em solar atmosphere} similarly by impact onto the dense layers below the corona] ({\bf process V}); it is lost [from {\em magnetospheres} (but not significantly from the {\em solar atmosphere})] to `infinity' by escape of fast neutrals from charge exchange ({\bf process V${\null}^{\prime}$}) and [from planetary magnetospheres and the solar atmosphere alike] by electromagnetic radiation ({\bf process V${\null}^{\prime \prime}$}). In the case of the Io torus at Jupiter, radiation (mainly UV) produced by atomic/molecular collision and excitation processes carries an amount of energy that is significant (possibly even dominant) for the magnetospheric energy budget.  Electromagnetic radiation from the [planetary] atmosphere (including auroral emissions) is not shown in Fig.\,\ref{fig:sumE}, the power involved being in general negligible on the scale of the magnetospheric energy budget; discussions of energy supply in the aurora usually refer to energy in the precipitating particles that excite the auroral emissions, not energy in the emissions themselves. [In contrast, for {\em solar flares} the emission from the magnetospheric counterpart of the 'atmosphere', namely the surface or photosphere, generally dominates the electromagnetic energy losses seen in impulsive events, and this process {V${\null}^{\prime\prime}$ is not negligible either when compared to the energy involved in the CME (process {III${\null}^\prime$).]

 (8) [In {\em magnetospheres},] {\bf Processes 0} extract energy from bulk flow but do not put it into the magnetosphere. For the solar-wind source, the net energy extracted from bulk flow as the solar wind is slowed down and forced to go around the magnetospheric obstacle represents the power expended in irreversible heating of solar wind plasma at the bow shock: when the plasma that has been compressed and heated at the bow shock expands far downstream to its initial (ambient solar-wind) pressure, it has a higher temperature (because of the increase of the entropy) and hence (by Bernoulli's law) a lower velocity. For the planetary-rotation source, the torque that extracts energy from rotation is transmitted by magnetic stresses which can act only as far as the bottom of the ionosphere; farther down, between the ionosphere and the planet, the torque must be transmitted purely by stresses in the neutral medium --- effective viscous stresses from velocity shear, accompanied in general by energy dissipation and thus heating of the neutral atmosphere. In both cases, the power involved may exceed by an order of magnitude the entire energy input into the magnetosphere. This is most obvious for Earth, where [the total force ${\mathrm F}_{\rm MP}$ exerted by the solar wind on the magnetopause]  exceeds [the total force ${\mathrm F}_{\rm MT}$ exerted on the field in the magnetotail] typically by a factor $\sim 10$; for Jupiter, it is suggested by the inference that, when ionospheric plasma slips relative to corotation, the neutral atmosphere very nearly moves together with the plasma, implying a large velocity shear below the ionosphere.  Processes 0 may thus constitute the largest energy dissipation processes in the entire interaction of the solar wind with a magnetized planet.'' For the {\em solar atmosphere}, there is a counterpart only in the heating of the chromosphere by flux emergence and by convective flows and associated waves.

Parallels to these processes can be found outside the present-day Solar System, and one in particular did occur in the earliest phases of the Solar System as it does in all young planetary systems: in Sect.~\ref{lh:4}, we encounter an environment that is fundamentally different from the Sun and the terrestrial planets as we know them today, but that nonetheless concerns a magnetosphere that is subject to instabilities driven by inflowing plasma: the accretion disk of a very young star and protoplanetary system, in which the stellar magnetosphere is stressed by the partially ionized matter orbiting in the disk that spirals into it. 

